Modeling Interval Trendlines: Symbolic Singular Spectrum Analysis for Interval Time Series

In this article we propose an extension of singular spectrum analysis for interval-valued time series. The proposed methods can be used to decompose and forecast the dynamics governing a set-valued stochastic process. The resulting components on which the interval time series is decomposed can be understood as interval trendlines, cycles, or noise. Forecasting can be conducted through a linear recurrent method, and we devised generalizations of the decomposition method for the multivariate setting. The performance of the proposed methods is showcased in a simulation study. We apply the proposed methods so to track the dynamics governing the Argentina Stock Market (MERVAL) in real time, in a case study that covers the most recent period of turbulence that led to discussions of the government of Argentina with the International Monetary Fund.

==> LaTeX/frametitle_memory.tex <==
% Keeps title from previous slide unless you ask him to change. Source: http://tex.stackexchange.com/questions/66274/re-using-the-title-of-the-previous-beamer-slide

\makeatletter
\def\beamer@checkframetitle{%
\begingroup
  \edef\temp{%
    \endgroup
    \noexpand\frametitle
    [\unexpanded\expandafter{\beamer@savedshortframetitle}]%
    {\unexpanded\expandafter{\beamer@savedframetitle}}%
  }
\temp
\@ifnextchar\bgroup\beamer@inlineframetitle{}}

\long\def\beamer@@frametitle[#1]#2{%
  \beamer@ifempty{#2}{}{%
    \gdef\insertframetitle{{#2\ifnum\beamer@autobreakcount>0\relax{}\space\usebeamertemplate*{frametitle
continuation}\fi}}%
  \gdef\beamer@frametitle{#2}%
  \gdef\beamer@shortframetitle{#1}%
  \global\let\beamer@savedshortframetitle\beamer@shortframetitle
    \global\let\beamer@savedframetitle\beamer@frametitle
}%
}
  \global\let\beamer@savedshortframetitle\@empty
    \global\let\beamer@savedframetitle\@empty

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> LaTeX/tikzBoxHighlight.tex <==
% This file can be used for constructing colorful boxes around objects such 
% text, using the command \highlight defined below. A minimal example is 
% \highlight<1>{Hello World!}

\usepackage{tikz}
\usepackage{xparse}    
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{calc}

\tikzstyle{every picture}+=[remember picture]
\tikzstyle{na} = [baseline=-.5ex]

\tikzset{
  invisible/.style={opacity=0,text opacity=0},
  visible on/.style={alt=#1{}{invisible}},
  alt/.code args={<#1>#2#3}{%
    \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} 
  },
}

\tikzset{
  background fill/.style={fill=#1},
  background fill/.default={white},
  fill on/.style={alt=#1{}{background fill}},
}

\tikzset{
  background draw/.style={draw=#1},
  background draw/.default={white},
  draw on/.style={alt=#1{}{background draw}},
}

\tikzset{
  background filldraw/.style args={#1 filled by #2}{draw=#1, fill=#2},
  background filldraw/.default=white filled by white,
  filldraw on/.style={alt=#1{}{background filldraw}},
}

\tikzset{highlighting/.style={
    append after command={
      \pgfextra{
        \path[rounded corners,
        background draw=blue,
        draw on=<#1>,
        overlay] ($(\tikzlastnode.south west)+(-0.015,-0.1)$) 
        rectangle ($(\tikzlastnode.north east)+(0.015,0.065)$);
      }   
    }
  }
}

\NewDocumentCommand{\highlight}{r<> m}{%
  \tikz[baseline=(A.base)] 
  \node[highlighting=#1,
  inner sep=0pt] (A) {#2};%
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

